Domain Analysis & Description - The Implicit and Explicit Semantics Problem

A domain analysis & description calculus is introduced. It is shown to alleviate the issue of implicit semantics. The claim is made that domain descriptions, whether informal, or as also here, formal, amount to an explicit semantics for what is otherwise implicit if not described.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{R. Laleau, D. M\'ery, S. Nakajima, E. Troubitsyna (Eds): Joint Workshop on\\ Handling IMPlicit and EXplicit knowledge in formal system development\\ and  Formal \& Model-Driven Techniques for Developing Trustworthy Systems.\\
EPTCS 271, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.271.1}{10.4204/EPTCS.271.1}}

